ScribeAgent: Towards Specialized Web Agents Using Production-Scale Workflow Data

Large Language Model (LLM) agents are rapidly improving to handle increasingly complex web-based tasks. Most of these agents rely on general-purpose, proprietary models like GPT-4 and focus on designing better prompts to improve their planning abilities. However, general-purpose LLMs are not specifically trained to understand specialized web contexts such as HTML, and they often struggle with long-horizon planning. We explore an alternative approach that fine-tunes open-source LLMs using production-scale workflow data collected from over 250 domains corresponding to 6 billion tokens. This simple yet effective approach shows substantial gains over prompting-based agents on existing benchmarks -- ScribeAgent achieves state-of-the-art direct generation performance on Mind2Web and improves the task success rate by 7.3% over the previous best text-only web agents on WebArena. We further perform detailed ablation studies on various fine-tuning design choices and provide insights into LLM selection, training recipes, context window optimization, and effect of dataset sizes.

==> figures/preprocessing.tex <==
\begin{verbatim}
def assign_element_id(all_tags):
    for i, tag in enumerate(all_tags[::-1]):
        tag["node"] = int(i)


salient_attributes = { "alt", "aria-role", "aria-label", ... }

def clean_tag(tag):
	for attr in list(tag.attrs):
		if attr in tag:
			if type(tag[attr]) == list:
				tag[attr] = " ".join(tag[attr])
			tag[attr] = str(tag[attr])[:32]
		if len(str(tag[attr])) > 32 and token_ratio(str(tag[attr])) < 2:
			del(tag[attr])
			continue

		if "script" in attr.lower():
			del tag[attr]
			continue

		if attr.lower() not in salient_attributes:
			del tag[attr]
			continue
		elif (tag[attr] == "" or tag[attr] == "none"):
			del tag[attr]
			continue
		
		if attr in tag:
			if tag.name == "iframe":
				if attr != "node":
					del tag[attr]
	tag = soup.prettify()
	return tag[:tag.find(">")+1]

valid_tags = { 'div', 'body', 'span', 'svg', 'input', 'img', 'p', ...}
code_elements_to_decompose = { 'style', 'script' }

def removing_tags(all_tags):
	count = 0
	for tag in all_tags:
		if tag.name in code_elements_to_decompose:
			tag.decompose()
		elif tag.name not in valid_tags:
			tag.unwrap()
	return all_tags

def generate_output(step_count, desc, kind, element_id, target_html):
	return f"{step_count}.\nDescription: {desc}\nAction: {kind}
 \nNode: {element_id}\nTarget: {target_html}\n"
\end{verbatim}

